Incorporating Uncertainty from Speaker Embedding Estimation to Speaker Verification

Speech utterances recorded under differing conditions exhibit varying degrees of confidence in their embedding estimates, i.e., uncertainty, even if they are extracted using the same neural network. This paper aims to incorporate the uncertainty estimate produced in the xi-vector network front-end with a probabilistic linear discriminant analysis (PLDA) back-end scoring for speaker verification. To achieve this we derive a posterior covariance matrix, which measures the uncertainty, from the frame-wise precisions to the embedding space. We propose a log-likelihood ratio function for the PLDA scoring with the uncertainty propagation. We also propose to replace the length normalization pre-processing technique with a length scaling technique for the application of uncertainty propagation in the back-end. Experimental results on the VoxCeleb-1, SITW test sets as well as a domain-mismatched CNCeleb1-E set show the effectiveness of the proposed techniques with 14.5%-41.3% EER reductions and 4.6%-25.3% minDCF reductions.

==> backuptable.tex <==

\begin{table}[t]
\caption{ Results are shown as EER/$\rm min$$\rm C_{primary}$.}
\centering
\centering
\caption{x-vectors were extracted from the 27 layer network}
\label{tab:exp0_try17n}
\begin{tabular}[t]{l|r|c|c|c}
\hline
     & system & Full cov & Diag W & Diag cov\\
\hline \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Vox1-o}}} 
                      &  ECAPA + PLDA  &   &   & \\
                      &  xi + PLDA     &   &   & \\
                      &  xi +UP-PLDA   &   &   & \\
\hline                      
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Vox1-h}}} 
                      &  ECAPA + PLDA  &   &   & \\
                      &  xi + PLDA     &   &   & \\
                      &  xi +UP-PLDA   &   &   & \\
\hline           
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{SITW}}} 
                      &  ECAPA + PLDA  &   &   & \\
                      &  xi + PLDA     &   &   & \\
                      &  xi +UP-PLDA   &   &   & \\
\hline           
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Cnceleb}}} 
                      &  ECAPA + PLDA  &   &   & \\
                      &  xi + PLDA     &   &   & \\
                      &  xi +UP-PLDA   &   &   & \\
\hline           
\end{tabular}
\label{tab:exp_lda}
\end{table}

==> tables.tex <==
\newcommand{\bb}[1]{\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=l]{270}{#1}}}}
{\renewcommand{\arraystretch}{1.1}
\begin{table*}[ht]
\centering
\caption{Performance of three ASV systems: ECAPA-TDNN x-vector and xi-vectors with PLDA, and xi-vector with uncertainty propagated PLDA on the four test sets: Vox1-o, Vox1-h and SITW core-core eval and CNCeleb1-E. UP1 and UP2 are UP-PLDA using the empirical covariance (square of std in xi*) and the posterior covariance, respectively.  
3 settings of the covariance matrices in PLDA are investigated.}    
\scalebox{0.77}{
\begin{tabular}{p{2.6cm}|p{1.2cm}p{1.2cm}p{1.4cm}*{2}{|p{1.2cm}p{1.2cm}p{1.35cm}}|p{1.4cm}p{1.4cm}p{1.5cm}}
    \hline
    \multirow{2}{*}{System} 
    & \multicolumn{3}{c|}{Vox1-o} 
    & \multicolumn{3}{c|}{Vox1-h}
    & \multicolumn{3}{c|}{SITW}
    & \multicolumn{3}{c}{CNCeleb}
    \\
    & Full cov & Diag W & Diag cov 
    & Full cov & Diag W & Diag cov 
    & Full cov & Diag W & Diag cov 
    & Full cov & Diag W & Diag cov
    \\
    \hline                    
    \hline                    
    x$(\mu, \sigma )$  
    & 2.08/0.239 &	1.31/0.169	& 1.44/0.184
    & 3.76/0.302 &	2.69/0.261	& 2.68/0.248
    & 2.24/0.200 &	1.78/0.184	& 1.86/0.179
    & 19.48/0.811 &	17.17/0.703	& 17.95/0.678\\
    %x$(\phi)$+UP$(\sigma)$   
    %&&& &&& &&&
    %\\
     xi$(\phi, \sigma )$
    & 2.10/0.214  & 1.35/0.141  & 1.42/0.158
    & 3.86/0.309  & 2.69/0.257  & 2.73/0.252
    & 2.33/0.204  & 1.69/0.178  & 1.86/0.177  
    & 19.94/0.767 & 17.34/0.702 & 18.38/0.678 
    \\
    xi + PLDA   
    &  2.30/0.223 & 1.47/0.181 & 1.49/0.166
    &  3.90/0.30  & 2.73/0.260 & 2.76/0.247
    &  2.30/0.201 & 1.80/0.174 & 1.91/0.178
    &  19.89/0.767& 17.32/0.713& 17.99/0.689 
    \\
    %xi$(\phi)$+UP$(\sigma)$   
    %&&& &&& &&&
    %\\
    xi$(\phi)$+UP$(\mathbf{L})$   
    & 1.07/0.169  & 0.98/0.145  & 0.99/0.129
    & 2.45/0.271  & 2.15/0.226  & 2.13/0.231
    & 1.73/0.177  & 1.69/0.169  & 1.80/0.170 
    & 13.84/0.795 & 11.34/0.694 & 13.18/0.714
    \\
    %xi$(\phi)$+UP$(\mathbf{L+\sigma})$  
    %&&& &&& &&&
    %\\
\hline                    
    %\bottomrule
   \end{tabular}}
    \label{tab:exp1}
    %\vspace*{-3mm}
    \label{tab:exp1}
\end{table*}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\renewcommand{\arraystretch}{1.1}
\begin{table*}[ht]
\centering
\caption{Performance of the proposed uncertainty in length scaling pre-processing and PLDA. SITW* and CNCeleb* are evaluations when not using mean adaptation for centralization.}
\scalebox{0.8}{
\begin{tabular}{c| c c c c c c}
    \hline
    Back-end  & Vox1-o   & Vox1-h  & SITW &  CNCeleb & SITW* & CNCeleb*
    \\
    \hline                    
    \hline                    
    PLDA            & 1.49/0.166 & 2.76/0.247 & 1.86/0.175 & 17.32/0.675 & 1.91/0.178 &17.99/0.689 \\
    LS PLDA         & 1.23/0.141 & 2.43/0.235 & 1.65/0.170 & 12.63/0.630 & 1.77/0.168 &15.04/0.676 \\
    UP-PLDA         & 0.99/0.129 & 2.13/0.231 & 1.77/0.167 & 10.81/0.652 & 1.80/0.170 &13.18/0.714 \\
    UP-LS UP-PLDA   & 1.01/0.124 & 2.18/0.224 & 1.59/0.167 & 10.16/0.608 & 1.59/0.166 &11.57/0.686 \\   
\hline                    
    %\bottomrule
   \end{tabular}}
    \label{tab:exp2}
    \vspace*{-3mm}
    \label{exp2}
\end{table*}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\renewcommand{\arraystretch}{1.1}
\begin{table*}[ht]
\centering
\caption{Performance of three ASV systems: 1) ECAPA-TDNN x-vector, 2) xi-vector with PLDA  and 3) with UP-PLDA on the four test sets: Vox1-o, Vox1-h, SITW core-core eval, and CNCeleb1-E. LS applied in the UP-PLDA system is UP-LS.
}    
\scalebox{0.8}{
%\begin{tabular}{l|p{1.2cm}p{1.4cm}*{2}{|p{1.2cm}p{1.35cm}}|p{1.4cm}p{1.5cm}}
\begin{tabular}{l|c c | c c| c c| c c}
    \hline
    \multirow{2}{*}{} 
    & \multicolumn{2}{c|}{Vox1-o} 
    & \multicolumn{2}{c|}{Vox1-h}
    & \multicolumn{2}{c|}{SITW}
    & \multicolumn{2}{c}{CNCeleb}
    \\
    & - & LS 
    & - & LS 
    & - & LS 
    & - & LS 
    \\
    \hline                    
    \hline                    
   xi%$(\phi)$
    & 1.49/0.166 &	1.23/0.141	
    & 2.76/0.247 &	2.43/0.235	
    & 1.86/0.175 &	1.65/0.170   	
    & 17.32/0.675 & 12.63/0.630
    \\
    xi+UP   
    & 0.99/0.129 &	1.01/0.124	
    & 2.13/0.231 &	2.18/0.224	
    & 1.77/0.167 &	1.59/0.167	
    & 10.81/0.652 & 10.16/0.608
    \\
    %xi$(\phi)$+UP$(\mathbf{L+\sigma})$  
    %&&& &&& &&&
    %\\
\hline                    
    %\bottomrule
   \end{tabular}}
    \label{tab:tab2}
    %\vspace*{-3mm}
    \label{tab:exp1}
\end{table*}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

